Predicting Long-Term Citations from Short-Term Linguistic Influence

A standard measure of the influence of a research paper is the number of times it is cited. However, papers may be cited for many reasons, and citation count offers limited information about the extent to which a paper affected the content of subsequent publications. We therefore propose a novel method to quantify linguistic influence in timestamped document collections. There are two main steps: first, identify lexical and semantic changes using contextual embeddings and word frequencies; second, aggregate information about these changes into per-document influence scores by estimating a high-dimensional Hawkes process with a low-rank parameter matrix. We show that this measure of linguistic influence is predictive of $\textit{future}$ citations: the estimate of linguistic influence from the two years after a paper's publication is correlated with and predictive of its citation count in the following three years. This is demonstrated using an online evaluation with incremental temporal training/test splits, in comparison with a strong baseline that includes predictors for initial citation counts, topics, and lexical features.

==> emnlp/results-online-evaluation.tex <==
\begin{tabular}{lrrrr}
\toprule

Publication Year & M1 & M2 & M3 & M4\\

\midrule

2000 & 0.819 & 0.825 & 0.842 & 0.843\\[4pt]

2001 & 0.886 & 0.892 & 0.894 & 0.894\\[4pt]

2002 & 0.913 & 0.919 & 0.916 & 0.921\\[4pt]

2003 & 0.892 & 0.900 & 0.897 & 0.903\\[4pt]

2004 & 0.888 & 0.902 & 0.898 & 0.901\\[4pt]

2005 & 0.913 & 0.920 & 0.919 & 0.923\\[4pt]

2006 & 0.919 & 0.928 & 0.930 & 0.933\\[4pt]

2007 & 0.911 & 0.919 & 0.917 & 0.920\\[4pt]

2008 & 0.883 & 0.888 & 0.889 & 0.890\\[4pt]

2009 & 0.898 & 0.903 & 0.899 & 0.903\\[4pt]

2010 & 0.895 & 0.902 & 0.897 & 0.899\\[4pt]

2011 & 0.879 & 0.884 & 0.886 & 0.889\\[4pt]

2012 & 0.885 & 0.895 & 0.894 & 0.894\\[4pt]

2013 & 0.909 & 0.913 & 0.913 & 0.916\\[4pt]

\\
\bottomrule

\end{tabular}

% generated at 06:24PM on June 17, 2022 by Sandeep from citation_predictions.ipynb

==> emnlp/tab-regression-statsmodels-results.tex <==
\begin{center}
\begin{tabular}{lclc}
\toprule
\textbf{Dep. Variable:}    & log\_residual\_cites\_z & \textbf{  R-squared:         } &     0.592  \\
\textbf{Model:}            &           OLS           & \textbf{  Adj. R-squared:    } &     0.591  \\
\textbf{Method:}           &      Least Squares      & \textbf{  F-statistic:       } &     1027.  \\
\textbf{Date:}             &     Fri, 17 Jun 2022    & \textbf{  Prob (F-statistic):} &     0.00   \\
\textbf{Time:}             &         16:19:52        & \textbf{  Log-Likelihood:    } &   -18595.  \\
\textbf{No. Observations:} &           19158         & \textbf{  AIC:               } & 3.725e+04  \\
\textbf{Df Residuals:}     &           19130         & \textbf{  BIC:               } & 3.747e+04  \\
\textbf{Df Model:}         &              27         & \textbf{                     } &            \\
\textbf{Covariance Type:}  &        nonrobust        & \textbf{                     } &            \\
\bottomrule
\end{tabular}
%\caption{OLS Regression Results}
\end{center}
\begin{center}
\begin{tabular}{lcccccc}
\toprule
                                                                       & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P$> |$t$|$} & \textbf{[0.025} & \textbf{0.975]}  \\
\midrule
\textbf{Intercept}                                                     &       0.9597  &        0.763     &     1.258  &         0.208        &       -0.536    &        2.455     \\
\textbf{C(lex\_influence\_irregular\_quantiles)[T.lex.inf(50<=c<75)]}  &       0.0182  &        0.012     &     1.565  &         0.118        &       -0.005    &        0.041     \\
\textbf{C(lex\_influence\_irregular\_quantiles)[T.lex.inf(75<=c<90)]}  &       0.0201  &        0.014     &     1.416  &         0.157        &       -0.008    &        0.048     \\
\textbf{C(lex\_influence\_irregular\_quantiles)[T.lex.inf(90<=c<100)]} &       0.0661  &        0.017     &     3.902  &         0.000        &        0.033    &        0.099     \\
\textbf{C(sem\_influence\_irregular\_quantiles)[T.sem.inf(50<=c<75)]}  &       0.0512  &        0.012     &     4.349  &         0.000        &        0.028    &        0.074     \\
\textbf{C(sem\_influence\_irregular\_quantiles)[T.sem.inf(75<=c<90)]}  &       0.0948  &        0.014     &     6.549  &         0.000        &        0.066    &        0.123     \\
\textbf{C(sem\_influence\_irregular\_quantiles)[T.sem.inf(90<=c<100)]} &       0.1946  &        0.018     &    10.920  &         0.000        &        0.160    &        0.230     \\
\textbf{log\_cites\_k\_z}                                              &       0.7215  &        0.005     &   139.641  &         0.000        &        0.711    &        0.732     \\
\textbf{topic\_0}                                                      &      -1.2448  &        0.768     &    -1.622  &         0.105        &       -2.749    &        0.260     \\
\textbf{topic\_1}                                                      &      -1.1377  &        0.769     &    -1.480  &         0.139        &       -2.644    &        0.369     \\
\textbf{topic\_2}                                                      &      -0.9923  &        0.768     &    -1.293  &         0.196        &       -2.497    &        0.512     \\
\textbf{topic\_3}                                                      &      -0.9905  &        0.768     &    -1.289  &         0.197        &       -2.497    &        0.516     \\
\textbf{topic\_4}                                                      &      -1.0729  &        0.768     &    -1.398  &         0.162        &       -2.577    &        0.432     \\
\textbf{topic\_5}                                                      &      -0.7424  &        0.769     &    -0.966  &         0.334        &       -2.249    &        0.764     \\
\textbf{topic\_6}                                                      &      -1.0581  &        0.767     &    -1.379  &         0.168        &       -2.562    &        0.446     \\
\textbf{topic\_7}                                                      &      -1.1300  &        0.769     &    -1.470  &         0.142        &       -2.637    &        0.377     \\
\textbf{topic\_8}                                                      &      -1.0188  &        0.769     &    -1.325  &         0.185        &       -2.526    &        0.488     \\
\textbf{topic\_9}                                                      &      -1.2802  &        0.768     &    -1.667  &         0.096        &       -2.785    &        0.225     \\
\textbf{topic\_10}                                                     &      -0.8916  &        0.768     &    -1.161  &         0.246        &       -2.397    &        0.614     \\
\textbf{topic\_11}                                                     &      -1.0067  &        0.769     &    -1.309  &         0.190        &       -2.514    &        0.500     \\
\textbf{topic\_12}                                                     &      -1.0782  &        0.768     &    -1.404  &         0.160        &       -2.584    &        0.427     \\
\textbf{topic\_13}                                                     &      -0.9839  &        0.770     &    -1.278  &         0.201        &       -2.492    &        0.525     \\
\textbf{topic\_14}                                                     &      -0.8309  &        0.768     &    -1.081  &         0.280        &       -2.337    &        0.675     \\
\textbf{topic\_15}                                                     &      -0.9231  &        0.769     &    -1.201  &         0.230        &       -2.430    &        0.584     \\
\textbf{topic\_16}                                                     &      -1.1400  &        0.766     &    -1.488  &         0.137        &       -2.642    &        0.362     \\
\textbf{topic\_17}                                                     &      -1.2204  &        0.768     &    -1.589  &         0.112        &       -2.726    &        0.285     \\
\textbf{topic\_18}                                                     &      -0.4980  &        0.776     &    -0.642  &         0.521        &       -2.019    &        1.024     \\
\textbf{topic\_19}                                                     &      -0.9384  &        0.768     &    -1.221  &         0.222        &       -2.444    &        0.568     \\
\bottomrule
\end{tabular}
\end{center}
\begin{center}
\begin{tabular}{lclc}
\toprule
\textbf{Omnibus:}       & 702.382 & \textbf{  Durbin-Watson:     } &     2.038  \\
\textbf{Prob(Omnibus):} &   0.000 & \textbf{  Jarque-Bera (JB):  } &  1174.867  \\
\textbf{Skew:}          &   0.323 & \textbf{  Prob(JB):          } & 7.60e-256  \\
\textbf{Kurtosis:}      &   4.027 & \textbf{  Cond. No.          } &      858.  \\
\bottomrule
\end{tabular}
\end{center}
